Stopping Criteria for Value Iteration on Stochastic Games with Quantitative Objectives

A classic solution technique for Markov decision processes (MDP) and stochastic games (SG) is value iteration (VI). Due to its good practical performance, this approximative approach is typically preferred over exact techniques, even though no practical bounds on the imprecision of the result could be given until recently. As a consequence, even the most used model checkers could return arbitrarily wrong results. Over the past decade, different works derived stopping criteria, indicating when the precision reaches the desired level, for various settings, in particular MDP with reachability, total reward, and mean payoff, and SG with reachability. In this paper, we provide the first stopping criteria for VI on SG with total reward and mean payoff, yielding the first anytime algorithms in these settings. To this end, we provide the solution in two flavours: First through a reduction to the MDP case and second directly on SG. The former is simpler and automatically utilizes any advances on MDP. The latter allows for more local computations, heading towards better practical efficiency. Our solution unifies the previously mentioned approaches for MDP and SG and their underlying ideas. To achieve this, we isolate objective-specific subroutines as well as identify objective-independent concepts. These structural concepts, while surprisingly simple, form the very essence of the unified solution.

==> 3_example.tex <==
\section{Overview}

\todo{Maybe merge the examples into the prelims; we don't want to illustrate our solution up front, I think, so we only exemplfiy previous work.}

Before we define the technical algorithm, we exemplify illustrate the arising problems as well as our solution.

\subsection{Anytime algorithm in MDPs}






\subsection{The additional complications of SGs}


\subsection{Extending the solution for reachability to other objectives}

In this paper, we generalize the idea of deflating SECs~\cite{KKKW18} to the other objectives. 
First, we exemplify the dual procedure of inflating, which is necessary for safety, total reward with $\star = \infty$ and mean payoff. 

Let us again consider the example in Figure~\ref{fig:lilBCEC}and let $q$ be a Minimizer state.
For simplicity, consider a safety objective with avoid-set $\{t\}$. 
The situation is dual: the lower estimate is initialized to 0 everywhere. Assume that by preprocessing we see that $s$ can never reach a bad state, and thus we set its safety-value to 1. Then $q$ has the choice between action $b$, leading to an estimate of 0, or action $c$, leading to an estimate of $\frac 1 3$. As $q$ is minimizing the safety-value, it picks $b$, and the lower estimate of $p$ and $q$ remains at 0 forever. However, staying inside the EC $\{p,q\}$ actually has a safety value of 1, as $t$ is never reached. 
Thus we have to \emph{inflate} the estimates to make the Minimizer leave the EC, as staying gives them the impression of a too low value. 
%The upper bound converges without additional procedures, as the Minimizer always picks the leaving action in $q$.

So we see that depending on what happens if we stay inside an EC, it can be necessary to deflate the upper bounds, reminding the Maximizer that staying does not reach the goal, or to inflate the lower bounds, reminding the Minimizer that staying is actually what Maximizer wants. 

Inflating and deflating greatly depend on the \emph{staying value}, the value we would get for staying inside an EC. In reachability, the staying value of $\{p,q\}$ is 0, as it does not contain the target; in safety, the staying value of $\{p,q\}$ is 1, as it does not contain an avoid state. 
Note that the cases typically handled by pre-processing are special cases of inflating and deflating: for reachability/safety, seeing that $s$ has a value of 0 respectively 1 is deflating/inflating an EC without exit to its staying value.

The relevance of the staying value becomes most apparent when considering mean payoff, as this objective does not depend on a finite prefix of a path as the other three, but rather depends on the part of the path that is repeated infinitely often. 
Thus, determining the value of staying in an EC is more complicated than for the other objectives, where staying always has a maximal value like 0, 1 or $\infty$ (for total reward with $\star = \infty$).

In fact, for mean payoff we perform an additional value iteration that calculates the $n$-step total reward, and use that to estimate the mean payoff, i.e. the staying value, in an EC\footnote{For simplicity, in this example we work with a single estimate of the staying value. The algorithm actually keeps a lower and upper estimate of the staying value, both of which converge in the limit.}. 

Then, the actual value iteration proceeds as follows: After initializing all lower estimates to 0 and all upper estimates to the maximum occurring reward, we perform a Bellman updates as usual to backpropagate information. However, this alone would never change the estimates.
Thus, we additionally inflate and deflate ECs that we guess to be SECs, setting the estimates either to the most promising exit or to the staying value, i.e. the additionally calculated mean payoff.

Consider the SG in Figure~\ref{fig:lilBCEC} with $q$ being a Minimizer state and let $\reward(s)=\reward(u)=\reward(p)=1$, and $\reward(q) = 2$. 
Using the total reward value iteration, we see that the staying value of the ECs $\{s\}$ and $\{t\}$ is 1, and the staying value of $\{p,q\}$ is 1.5.

The value iteration to obtain the mean payoff values starts the lower and upper estimate at 0 respecitvely 2 (the highest occurring reward).
In $s$ and $t$, as there are no exits, both estimates are de- and inflated to their staying value of 1.
A Bellman update decreases the upper estimate in $q$ to the estimate of action $c$. This yields $\frac 4 3$, since it still depends on the upper estimate of 2 in $q$. In the limit, it will correctly converge to 1. 
Note that here deflating does not affect the upper estimate, as there is no Maximizer exit and the staying value is higher than the estimate we obtained by Bellman updates. Deflating can never increase and inflating can never decrease an estimate.
The lower estimate remains at 0 after a Bellman update, because $q$ is under the illusion of getting 0 for staying in the EC. 
Inflating the lower estimate of $\{p,q\}$ to the minimum of the best exit of Minimizer (1) and the staying value of the EC (1.5) increases the lower estimate to the correct value 1. 

If $q$ is a Maximizer state, both deflating and inflating are necessary. Deflating realizes that the staying value of $\{p,q\}$ is higher than the best exit and sets the upper estimate to the correct value 1.5. 
It is necessary to also inflating to the staying value, because Bellman updates can only backpropagate the information that the best exit $(q,c)$ achieves a value of 1.

In summary, we see that in SGs collapsing does not work. Instead, we guess SECs and gradually deflate and inflate them, using objective-specific staying values. 


%
%
%\subsection{Total reward}
%
%For total reward, for simplicity let us assume that there are no positive cycles. This special case is handled in the technical sections. 
%%These can be handled separately a priori by detecting them and assigning estimate $\infty$ to all states that can reach them. Actually, not necessarily, because we might have remind Min that they have to leave some EC else they get infty.
%Under the assumption, we can calculate an over-approximation for the total reward as in~\cite{ensuring}. Then the situation is completely analogous to either reachability for the type $\star = c$ or safety for the type $\star = \infty$.
%
%Consider the SG in Figure~\ref{fig:lilBCEC} with target state $u$ and let $\reward(t)=2$ be the only positive reward. Additionally, assume that we calculated the safe over-approximation for the total reward as 15.
%For $\star=c$, assume that all states are Maximizer states. Then the upper estimate in $q$ will never decrease below 15, as $q$ believes staying in the EC by going to $p$ yields that value. We have to deflate the EC so that it depends on the exit and converges to the correct value.
%For $\star=\infty$, let all states be Minimizer states. Then the lower estimate in $q$ will always stay at 0, as the estimate of $p$ is 0. However, under these semantics, staying inside the EC and not reaching the target $u$ yields a total reward of $\infty$, so this estimate is too low and Minimizer has to leave the EC. Thus, we inflate the estimate to depend on the exiting action $c$.
%The third type $\star=0$ is also handled in the technical section and not exemplified here.



==> 4_algorithm.tex <==
\subsection{LATER STUFF}

\todo{MAXVAL MINVAL belongs to later chapter}
For convenience, we introduce the shorthands $\minVal(\Phi)$ and $\maxVal(\Phi)$, which refer to the lowest respectively highest possible value that can occur for an objective.
We sometimes omit $\Phi$ if we feel like it. \todo{find some consistency in when we use it and when we don't}
We have $\minVal = 0$ for all 4 objectives; $\maxVal = 1$ for reachability and safety; and
$\maxVal = \max_{s \in \allstates} \reward(s)$ for mean payoff.
For total reward, the definition of $\maxVal$ is more complicated: using $\infty$ would be correct, but value iteration is not able to get rid of $\infty$, see Example X in Appendix Y. \todo{Example: Figure~\ref{fig:lilBCEC}. If EC has $\ub=\infty$, even if we deflate to best exit, this depends on states in the EC, which have $\ub=\infty$, so it doesn't go away. So we need a way to estimate the highest possible value non-infinite value}
We have to use some rational number $\ub(\G)$ that is higher than the highest possible non-infinite total reward. Such a number can be computed by extending the techniques from~\cite{ensuring}. See \todo{Appendix Z} for details.




\section{Global approach: Reducing to MDP}\label{sec:MDP-view}

\begin{algorithm}[t]
	\caption{Bounded value iteration based on global reduction to MDP}\label{alg:MDP-view}
	\begin{algorithmic}[1]
		\Require 
		\Statex SG $\G$, Objective $\Phi$, initial state $\initstate$ precision $\varepsilon$
		\Ensure 
		\Statex Over- and underapproximations $\ub$ and $\lb$ such that $\ub \geq \val \geq \lb$ and $\ub(\initstate)-\lb(\initstate) \leq \varepsilon$
		\Procedure{$BVI_{MDP}$}{$\G$,$\Phi$,$\initstate$,$\varepsilon$}
		\Repeat
		\Statex \Comment{Recommender procedure}
		\State $x \gets \text{Bellman}(x)$ \Comment{Standard value iteration} \label{line:convergentVI}
		\State $\straa,\strab \gets $ optimal Maximizer and Minimizer strategy inferred from $x$ \label{line:infer}
		\medskip
		\Statex \Comment{Compute bounds}
		\State $\lb \gets \max(\lb, \val(\G^\straa)) $ \label{line:lb}
		\State $\ub \gets \min(\ub, \val(\G^\strab)) $ \label{line:ub}
		\Until{$\ub(\initstate)-\lb(\initstate) \leq \varepsilon$}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%	Old stuff below	%%%%%%%%%%%%%%%%%%%%%%%

In the first subsection, we give an overview of the algorithm and prove its correctness and termination based on assumptions about a subprocedure which we call \emph{recommender procedure}. Then we show that the assumptions about this procedure are indeed justified in the second subsection.
\todomaxi{I don't like the phrase ``recommender procedure''. I still use it to emphasize that we can use anything with certain properties, and to show how general the algorithm is. Open for better names for the procedure. Note also that I differentiate procedure and algorithm, for the recommender thing and the whole thing.}
\todot{abstract VI should be explained here, too}


\subsection{Algorithm}

As shown in Example \textcolor{red}{X}, the solution for reachability works as follows: 
i) fix some strategy of Minimizer that looks promising given the current knowledge, but might be suboptimal. ii) Find MECs in the MDP induced by this strategy. iii) Deflat the upper estimate of all MECs by considering only the best exits from the MECs.

We generalize this by observing that whenever we fix any strategy of Minimizer, the values in the induced MDP are an over-approximation of the values in the SG. 
Intuitively, this is because the optimal strategy of Minimizer could play better actions and thus decrease the value; but the value of the SG cannot be higher, because Minimizer can certainly restrict it to the values in the MDP by playing the given strategy.
Dually, fixing any Maximizer strategy and solving the induced MDP gives an under-approximation of the values in the SG. 
Using these two observations, we can add a stopping criterion to any procedure that recommends a sequence of strategies and converges so that it eventually recommends the optimal strategies. 
In particular, we can instantiate the recommender procedure with the existing convergent value iteration algorithms.
The way to do that is summarized in Algorithm~\ref{alg:abstract}. 
Intuitively, for any pair of strategies that recommender procedure offers, the algorithm computes the values in the MDPs induced by fixing one or the other strategy, thereby obtaining over- and under-approximations of the value. 
Since by assumption the optimal strategies are eventually recommended, the approximations converge in the limit.
\todot{shorten by using sup inf notation. See comment in tex}
%hier könnte man auch einfach sowas sagen wie die value des games ist ja sup inf bzw inf sup, wenn man das eins fixiert dann gibt das natürlich einen lower / upper bound auf den sup / inf wert. also sowas wie V* = sup_s inf_t G^s,t >= inf_t G^s',t


For a really abstract algo, see Appendix~\ref{app:abstractAlgo}.





\begin{remark}[Monotonicity of Algorithm~\ref{alg:abstract}]\label{rem:monotonic}
	Note that Algorithm \ref{alg:abstract} is not monotonic, as we make no assumption that the sequence of strategies output by the recommender procedure is monotonically increasing.
	However, it is easy to modify the algorithm in order to obtain the desirable property that the estimates generated by Algorithm~\ref{alg:abstract} are monotonic.
	One has to initialize $\lb$ and $\ub$ to estimates that are certainly under- respectively over-approximations. This can be done e.g. by using $\minVal$ and $\maxVal$ as initial estimates.
	Then we can modify Lines \ref{line:lb} and \ref{line:ub} as follows:
	\begin{align*}
		\lb &\gets \max(\lb,\text{solution of Minimizer-MDP } \G^\straa)\\
		\ub &\gets \min(\ub,\text{solution of Maximizer-MDP } \G^\strab)
	\end{align*}
	where $\max$ and $\min$ take the pointwise maximum respectively minimum from the vectors. 
\end{remark}



\subsection{Recommender procedures}

\todomaxi{I know the headings are horrible, they are just there to make the structure obvious.}

To complete the abstract algorithm, we prove that for every objective there are recommender procedures that satisfy the assumptions.
We first consider value iteration based procedures, split into the finite-prefix dependent objectives, i.e. all except mean payoff, and then mean payoff.
Then we consider strategy iteration based procedures.

\subsubsection{Finite-prefix dependent value iteration based recommender procedures}

Convergent value iteration procedures exist for reachability~\cite{condonAlgo} and total reward~\cite{SGreward}.
For safety, the procedure exists by the duality to reachability, i.e. instead of considering a safety objective of Maximizer, one can switch the players and have Minimizer maximize a reachability objective. The safety value can be obtained as 1 minus the reachability value. \todot{Shorten the thing on safety, it disturbs the flow. Maybe some Krish paper did it?}

We can obtain strategies from a given vector of values by picking the state with the best current estimate in every state (where best is highest for Maximizer and lowest for Minimizer states). In case of ties, we have to ensure that we do not pick actions that cycle inside an EC. For example in Figure 1, we must not pick action b for state q, even though both action b and c have the same value. \todo{ensure this fits the Figure after modifying the example}
A way to ensure that we pick actions that make progress is to use an attractor construction similar to \todo{cite Krish sec 5.3}: perform a backwards breadth-first search from the target states and remember in which iteration a state was discovered. In case of equality between actions, pick that action that leads to a state that was discovered in the earliest iteration. 
In the example, s is discovered in the zeroth iteration, while r is discovered in the second. Thus action c is prefered to action b.
Note that states that are not discovered by the backwards breadth first search (such as t in the example) have no path to the target. Thus they have value 0 and their strategy is irrelevant, any of the available actions can be used.
\todot{This approach doesn't work for TR. Rather ``save arg-max, which gives witness for free'' M: It works if we first exclude infty. Generally: Maybe move this whole stuff to prelims and cite and handwave}


\begin{lemma}[Value iteration based recommender procedures for finite-prefix dependent objectives]
	For each of the objectives reachability, safety and total reward of type $\star=c$ or $\star=\infty$ there exists a convergent value iteration algorithm.
	Further, in every iteration one can infer strategies from the intermediate results of value iteration.
	Eventually, the inferred strategies are optimal.
\end{lemma}
\begin{proof}
	\todo{We have to either make this more formal or less detailed. I didn't want to do this in a lot of detail, since I guess most of it is common knowledge. Maybe move most of the stuff about finite prefix dependent objectives to appendix?}
We know from previous work that the VI algorithms converge in the limit. 
Thus, whenever two actions have a different value, eventually we will see this for all future iterations, and thus we can pick the better one.
When actions have the same value, an optimal strategy can pick any of them, provided it does not loop inside an EC. An action inside an EC can never look better than the exit, so we certainly pick the right action eventually.
\end{proof}


\subsubsection{Mean payoff value iteration based recommender procedure}

For mean payoff, we first have to extend the proof that it works from MDP to SG.
Note that when calculating the mean payoff, we assume that game is aperiodic, as there is a standard transformation to get this. \todot{Add details here, refer to appendix}
\todot{Mean payoff primer, description of MDP procedure, description of modifications for SG, proof of convergence, description how to obtain strategies, proof of assumptions about procedure}

\subsubsection{Strategy iteration based recommender procedures}
We can also use the schema of Algorithm \ref{alg:abstract} to obtain anytime bounds for strategy iteration.
\todo{describe SI already in prelims}

SI gives a sequence of strategies for one player that converges to an optimal strategy. We can always take the counter-strategy as the current strategy of the other player, thereby obtaining a sequence of strategy tuples. 
Since SI finds an optimal strategy of one player, the final best response is also an optimal strategy. Thus, using SI also satisfies the assumptions on the recommender procedure.






\section{Refining the abstract algorithm}\label{sec:refine}

There are two ways in which the abstract algorithm can be refined for value iteration recommender procedures:
Firstly, depending on the objective, we can link the VI to the computation of L or U, simplifying the computation of the stopping criterion.
Secondly, to avoid solving a complete MDP in every iteration for the computation of L and U, we can instead use heuristics.
Using both of these refinements, we can obtain the original algorithm from \cite{KKKW18}, its optimization from \cite{widestPaths}, as well as similar algorithms for the other objectives that are potentially more practical. 


\subsection{VI: Objective specific refinement}
Reach/TRc: VI is actually a lower bound, so we can use it as L.
Safe/TRinf: VI is actually an upper bound, so we can use it as U.
MP: VI is independent, as it is prefix independent, so we really need to keep L and U separate.
\todo{Need good way to write this down; sth that makes clear which variables coincide etc.}

\begin{lemma}
	Replacing the $\lb$ computation with $x$ for reach/TRc or replacing the $\ub$ computation with $x$ for safe/TRinf, Algorithm \ref{alg:abstract} still is correct and terminates.
\end{lemma}

Note that this also eliminates the cases where we fix a Max strat according to L or a Min strat according to U, which was kinda unintuitive. (Maybe noone else cares, but I'm glad about this)\todot{Tobi disagrees}

\subsection{VI: Approximate solving of the MDPs}
Instead of solving the whole MDP for computation of L or U, we can use a heuristic as follows. Note that we describe it for $\ub$, as this will lead to deriving the algorithm from \cite{KKKW18}; however, you can do the exact same thing for $\lb$, replacing $\strab$ with $\straa$ and $\max$ with $\min$.

Replace the line ``$\ub \gets $ solution of $\G^\strab$''
with 
``$\ub \gets \heur(\G^\strab,\ub)$. 
(note we could again add the $\max$ with previous $\lb$ to make it monotonous, see Remark \ref{rem:monotonic}). 

The heuristic gets an MDP (the SG with one strategy applied) and the previous estimate.
The only thing we require of the heuristic is that, given a valid upper estimate $\ub$, we have
$\lim_{i \to \infty} \heur^i(\G^\strab,\ub) = \val(\G^\strab)$, i.e. applying the heuristic converges to the true value of the MDP \todo{not type correct, since heur has two parameters, need to rephrase}.

\begin{lemma}
	If we replacing the ``solve'' in Algorithm \ref{alg:abstract} with $\heur$ as just described, the algorithm still is correct and terminates.
\end{lemma}
\begin{proof}
	We still have the assumption that we eventually get a pair of optimal strategies infinitely often from the recommender procedure.
	At that point, the upper bound computation simplifies to repeatedly applying the heuristic $\heur$ to $\G^\strab$ and $\ub$. By the requirement of the heuristic, this converges to $\val(\G^\strab)$.
	Dually the same for $\lb$.
\end{proof}

\subsection{VI: Concrete algorithm for finite-prefix dependent objectives}

It remains to describe heuristics $\heur$ for all objectives that satisfy the requirement.

For reachability, safety and total reward, a convergent VI algorithm for solving MDPs works by detecting and collapsing MECs and then applying Bellman updates to the estimates~\todo{cite sth}.
To perform just a single step of this algorithm, we have to collapse MECs in the MDP, apply a single Bellman update, and then revert the collapsing. 
This way, all states in a MEC now have the same estimate, as they were grouped together. The value they have is that of the $\bE$ from the MEC. 
\todot{Tobi commented: ich würde von dem collapsing weggehen, das ist nicht essentiell, das ist nur ne möglichkeit wie man sich das einfach vorstellen kann. man muss das MDP nicht modifizieren damit man die updates hinbekommt (-> bestExit analyse). also vielleicht vielleicht sowas wie "modified Bellman update"?}

This is correct, as it is just a step of the correct solution algorithm for MDPs.
This satisfies the requirement for the heuristic, as repeatedly applying it is the same as collapsing and then just applying Bellman updates until convergence.
In other words: Uncollapsing every step does not hinder the correctness or convergence of the original algorithms.

Note that now we obtain the algorithm of \cite{KKKW18}:
The lower estimate is computed by normal value iteration, as by Lemma sth we showed that this is possible. 
For the upper estimate, the deflating procedure first fixed a Minimizer strategy according to $\lb$, as we do here, then computed the MECs in the resulting MDP (calling them SECs), as we do, and then decreased the upper estimate for all states in the MEC to that of the $\bE$. This is equivalent to collapsing the MEC, doing one Bellman update, and then uncollapsing the MEC. For all states that are not part of a MEC, on Bellman update is executed in both algorithms. The one from \cite{KKKW18} just separates the cases whether a state is part of a MEC in the MDP (deflating) or whether it is not (normal Bellman update), while our algorithm first collapses, does the Bellman update everywhere, and then uncollapses.
The algorithm works exactly the same for total reward with $\star = c$.

For safety and total reward with $\star = \infty$, the heuristic is necessary for the lower bound. Thus, to mirror the procedure of deflating, we can introduce \emph{inflating}:
It works by fixing a Maximizer strategy, finding MECs in the resulting MDP (guesses of the SECs) and increasing the lower bound to the best Minimizer exit (or 1, if there is none). This is exactly the same as collapsing the MEC and applying one Bellman update.

\subsection{VI: Concrete algorithm for mean payoff}

\todomaxi{This section can use the information we gave when defining the recommender procedure.}

For mean payoff, the situation is more complicated in two ways: Firstly, as the convergent VI aggregates total reward, it only implicitly calculates mean payoff and cannot be used as upper or lower bound. 
Secondly, the algorithm for solving MDPs is not only collapsing and Bellman updates, but it additionally needs to compute the values of staying inside the MECs, and only afterwards can perform a weighted reachability. 

Thus, a heuristic $\heur$ needs a way to be informed about the staying values. It has a third parameter which is the current total reward that was computed by the convergent VI. 
Using that, we can infer upper and lower bounds on the staying value of every MEC in the MDP, and thus for both upper and lower bound computation we have correct estimates available.

The algorithm for fully solving an MDP collapses and then uses weighted reachability, initializing the collapsed states with their staying value.
To break this down to a single step, we have to collapse and do Bellman update as previously, but additionally, we have to include the staying value. 
We have
$\ub(s) = \min(\ub(s),\max(\bE_\ub^\Box(X), \stayVal(X)))$ and 
$\lb(s) = \max(\lb(s),\min(\bE_\lb^\circ(X), \stayVal(X)))$.
(note that in the $\bE$, circ and box are not necessary, as we are talking about an MDP where all states belong to that player)

Note that this definition of inflating and deflating also suits the other objectives for suitable definition of staying value (insert definition of staying value here).

Aggregating all the points we just made, we can provide the following algorithm which stays inside the SG world and doesn't require full MDP solving. \todo{Not sure we want this, but it actually naturally developed while writing}
Note that the calculation of $\stayVal(X)$ for mean payoff requires to have a total reward value iteration in the background. 


\subsection{VI: Relation to widest paths}
The widest path algorithm from \cite{widestPaths} is the same with a different heuristic. They are actually closer to our abstract algorithm: They explicitly construct the MDP under currently optimal Minimizer strat, and then they turn it into a weighted graph that over-approximates the MDP. By solving the widest path problem on the weighted graph, they don't locally apply a Bellman update to the collapsed MEC, but instead globally solve the weighted graph. As the upper bound becomes more precise over this process, the upper estimate converges.

This heuristic can also be used in our algorithm: replacing the MDP solving by "construct weighted graph and then solve that". 

\todomaxi{We probably want to talk about this sooner; then we could directly derive the widest path for all algorithm, not the one that I gave. As you may have noticed, for the whole Section \ref{sec:refine} I am not sure about the structure.}


\subsection{Refining the SI version}

When using SI as recommender procedure, a step of SI always solves the Minimizer-MDP $\G^\straa$, so the computation of $\lb$ is built into the recommender procedure.
However, the computation of $\ub$ is not used for the recommender procedure at all\footnote{We could of course also get a sequence of Minimizer strategies. Then $\ub$ is part of the recommender procedure and $\lb$ is not used}.

We are actually computing alternating best responses of both players; we could leverage information from both MDPs.
However, \cite{condonAlgo} showed that alternatingly taking best responses can lead to cycling behaviour and doesn't converge. 
However, we feel like we should be able to make this work. Maybe it requires adding the monotonicity thing as in Remark \ref{rem:monotonic}. That way, information is not discarded between iterations, and we can't cycle, hopefully.
Tobi is of the opinion that even this might not be needed. 

Note that, if we were to take alternating best responses, this would go back to the intuitive way of getting the next Max-strat from an over-approximation, not from an under-approximation as is usual in SI. \todomaxi{Again, maybe noone cares about this, but it feels more natural to me and maybe we can make such an argument.}

\todo{Actually develop the algorithm and prove it}

\section{Things we also want to mention that right now don't fit the story}



These concepts of best exit and staying value are so important, because they suffice to determine whether an EC will hinder the convergence of normal value iteration and needs deflating or inflating.
The following observation is a generalization of~\cite[Lemma 1]{KKKW18}.

\begin{theorem}[Problematic end components]\label{lem:pEC}
	Let $X$ be an EC. 
	If the best exit of Minimizer yields a value higher than the best exit of Maximizer and the staying value, i.e.
	$\max(\stayVal(X),\bE^\circ_\val(X),\bE^\Box_\val(X)) = \bE^\circ_\val(X)$,
	then for every $m$ with  $\bE^\circ_\val(X) \geq m \geq \max(\stayVal(X),\bE^\Box_\val(X))$ there is a solution to the Bellman equations which on $X$ is constant and equal to $m$.
	
	Dually, if the best exit of Maximizer yields a value lower than the best exit of Minimizer and the staying value, i.e.
	$\min(\stayVal(X),\bE^\circ_\val(X),\bE^\Box_\val(X)) = \bE^\Box_\val(X)$, 
	then for every $m$ with  $\bE^\Box_\val(X) \leq m \leq \min(\stayVal(X),\bE^\circ_\val(X))$ there is a solution to the Bellman equations which on $X$ is constant and equal to $m$.	
\end{theorem}
\begin{proof}
	Intuitively, both players prefer $m$ to using their exits. Thus, it is a fixpoint of the Bellman equations, as both players do not depend on their exits, but remain under the illusion they can achieve $m$ by staying.
\end{proof}

This lemma characterizes all the situations in which we have to deflate/inflate. \todo{Might actually prove an if and only if, i.e. if this is not the case, everything works out}

Deflating and inflating are defined in Line~\ref{line:defl} respectively~\ref{line:infl} of Algorithm~\ref{alg:general}.
They address exactly the problem that Lemma~\ref{lem:pEC} points out.
For deflating, if $\bE^\circ_\val(X)$ is the highest of the three relevant values, the upper estimate remains at that high value, even though Minimizer will never take the exit. So we deflate the upper estimate down to something realistic, the maximum of the staying value or the best exit of Maximizer.
For inflating, we have the dual situation.

\todo{add running examples?}

\begin{remark}[Algorithm with an oracle]
	Even if we had an oracle to tell us all the SECs of the game, we could not simplify the second step of the approach using \emph{collapsing}~\cite{atva,HM18}.
	In reachability, it is possible to collapse SECs into a single Maximizer state and only keep all the exiting actions of Maximizer.
	However, this only works because the staying value in reachability is trivially 0 and thus irrelevant.
	Without knowing the relative order of the staying value as well as the values of the best exits of Maximizer and Minimizer, it is not possible to collapse a SEC into a single state, because it is not clear to whom the state belongs, and whether we keep the exits of Maximizer, Minimizer, or only a self-loop with the staying value.
\end{remark}

Note that for total reward, we have two choices of how to look at it: Either we first find the states that can reach a positive cycle, assign infinite reward and remove them from consideration (which keeps proofs nice and easy), or we see these infinite cycles as a special case of inflating. The check is whether the current EC has a positive reward in it. 
Second thing seems more elegant; practically I'm not sure which one is better; first thing is easier to prove. For second thing we need to make sure that $\min_\emptyset = \infty$ in total reward.




==> 5_proofs.tex <==
\section{Technical details/proofs}

\todomaxi{I will go through the paper and aggregate Lemmata that we need proven and put their statements here. Then Tobi and I can insert the proofs. }


%\begin{algorithm}[h]
%	\caption{MP-VI}\label{alg:MPVI}
%	\begin{algorithmic}[1]
%		\Require 
%		\Statex SG $\G$
%		\Ensure 
%		\Statex $\epsilon$ precise values for all states/initial state.
%		\Procedure{\textsf{MP-VI}}{$\G$}
%		\While {Stopping criterion not met}
%			\State Do a step of MP-VI
%			\State Guess SECs according to current local min strategy
%			\State Construct weighted quotient game (replacing SECs with ECs, weighted reachability)
%			\State Check weighted quotient game for conflicts: If guess was incorrect, abort. If guess was correct, backpropagate current information for guaranteed interval.
%		\EndWhile
%		\EndProcedure
%	\end{algorithmic}
%\end{algorithm}

%The algorithm may also first do a lot of MP-VI. The guessing must happen infinitely often, but can also happen only every $n$ steps or when the span norm looks good everywhere. Also, it might pay off to use the topological variant of VI. 
%
%Note that solving the weighted quotient game needs the staying value buisness that we currently don't have written down.
%However, as currently we can't even solve a single bottom MEC, that's not the first point on the list.

\subsection{Proof ideas for MP}
\todo{Proceed with care, unordered and possibly outdated}
\begin{lemma}\label{lem:conv}
	VI for MP in games and converges in the limit.
\end{lemma}
\begin{proof}
	Extend Puterman Theorem 9.4.1. I didn't find this proof in literature; for total reward, we CFK+13 (Automatic verification of competitive stochastic systems) Appendix B. However, they exclude the possibility of infinite rewards by detecting and removing them, and MP only cares about infinite rewards... 
	Still, should be reasonably straightforward.
	We still have that the lower iteration computes the n-step total reward, I guess. Thus, for inf-ECs we won't get to the right total reward number, as it is inf. However, for MP, converging towards inf at the right speed is acceptable. Just divide by number of iterations and happy. 
	Think about how bad it is if we have different number of iterations within the same MEC.
	
	Remember to handle the aperiodic buisness and so on. 
\end{proof}

\begin{lemma}
	Given correct guesses of the SECs, everything is easy.
\end{lemma}
\begin{proof}
	Similar to ACD+17. Differences: 
	1. SECs instead of MECs, as the value comes from those. 
	2. Need staying value to make sure non-bottom ECs are treated correctly. Maybe automatically in the quotient construction (since they have the staying action, which is basically what deflate does)
\end{proof}

%\begin{lemma}
%	Our procedure for whether SECs are guessed correctly is sound and complete.
%\end{lemma}
%\begin{proof}
%	It is not.
%	BSCC has problem in Figure 1.
%	For SEC, not sure how to prove it.
%	
%	Idea of procedure: Fix Min strat according to local values, then check that within the MEC the lowest lower bound is not ignored or sth?
%	Assume we guessed incorrectly, then the action leading to better SEC certainly has lower value, because...?
%	Maybe running until span norm is small helps?
%\end{proof}

\begin{theorem}
	The whole thing works, i.e. converges towards true value and gives bounds on the way.
\end{theorem}
\begin{proof}
	As long as SECs are guessed wrongly, we refute the guesses and nothing bad happens.
	The SECs are eventually guessed correctly (or rather correctly enough, since we might never detect equality, but noone cares).
	Given a correct guess, the upper and lower estimates are propagated correctly (upper and lower estimate is equal to mean of occurring things plusminus half the span norm; equivalently, we could run until span norm is small and then propagate those things).
\end{proof}

%\section{All the ideas to make it more sensible/efficient}
%As we said earlier, do the special stuff only every $n$ steps.
%
%Topological, i.e. first solve later MECs, then use those results. If necessary, improve later MECs.
%
%BRTDP might work, but currently hard to think about.
%
%Can always use lowest and highest appearing mean payoff as lower and upper bound for MEC, and thus already do sth with it. The SEC buisness can make these values finer.

The staying value is correct:
For an EC that is a BSCC under optimal strategies, the value always stays between the highest and lowest occurring estimate for this EC.
\todo{proper proof}

Deflate/Inflate is sound (given correct L and U as input):
If we pick sth that is BSCC under optimal strategies, it is ok by previous lemma.

If we pick sth that is not BSCC under optimal strategies, then at least one of the players has an action with a better value available. As the given L and U are correct, deflate/inflate will not change the value beyond the L/U of that leaving action with a better value (and thus better L/U).

\subsection{For Tobi}
\todo{Tobi can write his proof ideas etc. here, and git will detect that it is its own section and not have conflicts}

==> 6_discussion.tex <==
\section{Discussion}

\subsection{Complexity}
Proof here. Should be EXPTIME everywhere. Needs at least EXPTIME (Kiefer et al. 19) and at most EXPTIME (even for the two VIs in MP).

\subsection{Comparison to other algos}
Discuss relation to other existing algos, e.g. say that previous approach of transformation was not promising and we are first anytime with precision guarantees before EXP many steps.
Could also set into context with approaches for MDPs (collapsing based), and say that they follow the same idea, just different (simpler) treatment of ECs.
(take care that the discussion does not overlap with the related work section in intro too much)


==> 9a_old_strats.tex <==
\subsection{Exemplifying the problem}

We start by illustrating the idea and the difficulty on an example.
Intuitively, a strategy just plays an action which is optimal according to the current approximants. 
However, this might not be sufficient, as the following counter-example shows.

\begin{figure}[t]
	\vspace{-1em}
	\centering
	\begin{tikzpicture}
		%little BCEC with loop
		\drawdummy (init) at (0,0) {};
		\drawbox (p) at (1,0) {$\mathsf{s}_1$};
		\drawbox (q) at (1,-2) {$\mathsf{s}_2$};
		\drawbox (1) at (5,-1) {$\mathsf{1}$ };
		
		\draw[->] (init) to (p);
		\draw[->]  (p) to[bend left] node [midway,anchor=west] {$\text{stay}_1$}(q) ;
		\draw[->]  (q) to [bend left] node [midway,anchor=east] {$\text{stay}_2$} (p);
		\draw[->]  (p) to node [midway,anchor=south] {$\text{exit}_1$} (1);
		\draw[->]  (q) to node [midway,anchor=north] {$\text{exit}_2$} (1);
		\draw[->]  (1) to [loop right] node [midway,anchor=west] {} (1) ;		
	\end{tikzpicture}
	\caption{An example of an $SG$ (also MDP) where following optimal actions is not necessarily an ($\varepsilon$-)optimal strategy.
	}
	\label{fig:strat-CE}
	\vspace{-0.5em}
\end{figure}

Consider the SG (that also is an MDP) from Figure~\ref{fig:strat-CE}.
% with three Maximizer states, $\mathsf{s}_1$, $\mathsf{s}_2$ and $\target$. Both $\mathsf{s}_1$ and $\mathsf{s}_2$ have two actions: \emph{stay}, which surely transitions to the other $\mathsf{s}_i$; and \emph{exit}, which surely transitions to the target. 
After one update we have $v_1(\mathsf{s}_1) = v_1(\mathsf{s}_2) = 1$ and $v_1$ is equal to the value. Thus, for both $i=1$ or $i=2$, we have $\argmax_{a \in \Av(\mathsf{s}_i)} v_1(\mathsf{s}_i,\action) = \{\textit{stay},\textit{exit}\}$.
Both actions are indeed optimal, as after playing \emph{stay}, the other state still can reach reach the target with probability 1. However, using the strategy that in both states picks the \emph{stay}-action results in probability 0 to reach the target.
Intuitively, the problem is that picking optimal actions only guarantees that they are one-step optimal, but does not ensure that the target is actually reached in the end.
Thus, in order to obtain optimal strategies, we additionally have to ensure that the strategies ``make progress'' towards the target.

A way to achieve this would be to randomize over all optimal actions; however, this is suboptimal, as theoretically it needs the additional power of randomization and practically the strategy has a chance of cycling unnecessarily by using the actions that stay instead of making progress.

In~\cite[Remark 10.104]{DBLP:books/daglib/0020348}, the authors observe that $v_i$ corresponds to the $i$-step-bounded reachability probability (for MDPs, but the argument extends to SGs). 
They suggest that a strategy obtaining this value can be generated by choosing an optimal action according to $v_i$ in the first state, then according to $v_{i-1}$ in the next step and so on.
In the previous example, for all $i>1$, both \emph{stay} and \emph{exit} are optimal, while for $i=1$ only \emph{exit} is optimal. Thus, this strategy ensures that the target is reached. 
However, note that this strategy requires memory as well as knowledge of all intermediate results $v_i$. 

We need to derive \emph{memoryless deterministic} optimal strategies in order to apply them in Algorithm~\ref{alg:MDP-view}.
We describe how to so, first in detail in the reachability setting and then pointing out the differences for the other settings.
%We now describe a way to obtain memoryless deterministic optimal strategies for Maximizer and Minimizer, using the sequence of value vectors generated by value iteration.
%Thus we provide a convergent strategy recommender which derives strategies from classical value iteration.

\subsection{Reachability}

\subsubsection{Assumptions}

For a vector mapping states to value $x$, we use the notation $x(s,a) \eqdef \sum_{s'\in\states} \trans(s,a,s') \cdot x(s)$ to denote unfolding the Bellman equations for one step with action $a$.

We are given a sequence of value vectors $x_i$ as computed by classical value iteration. This means we initialize $x_0$ to 1 in target states and to 0 everywhere else and then apply Bellman updates according to Equation~\ref{eq:bellman}.
We know from e.g.~\cite{DBLP:journals/iandc/BrazdilBKO11} that for all $i \in \Naturals_0$
\begin{enumerate}
	\item the approximants are correct, i.e.\ $x_i \leq \val$.
	\item the targets-approximants are precise, i.e.\ for all $s \in \fstates$ we have $x_i(s) = 1$ 
	\item unfolding the Bellman equation for one step can only make the approximants more precise, i.e. for all $s \in \states$
	\[
		x_i(s) \leq \opt_{\action \in \Av(s)} x_i(s,a).
	\]
\end{enumerate}

Moreover, we know that value iteration converges.
Thus, there exists a $j\in \Naturals$ such that for all $i \geq j$ we have that for all states $s \in \states$, only truly optimal actions are optimal according to the approximants, formally
\[
	\opt_{\action \in \Av(s)} x_i(s,a) = \opt_{\action \in \Av(s)} \val(s,a)
\] 

\subsubsection{Following only the approximants}
We define the strats as
pick opti for Min

Lemma follow approx for finite time is opt
Lemma: eventually min strat is optimal 

opti-Attractor for Max.
Lemma: eventually this is optimal strat

\subsubsection{Convergent strat recommender}
Combining Lemma X and Y, we have shown how to obtain strategies from VI for reachability such that eventually both strats are optimal in every step.

\subsection{Safety}
For the safety objective, value iteration starts from above, i.e.\ 0 in avoid states and 1 in all other states.
Then, we converge from above. 
The assumptions change as follows.
Lemma W is the same, since it only needs assumption (c), which is unchanged.

A Maximizer strat can remain, and by analogue of Lemma X it is optimal. The proof differs in that now the x-th term is 0 or sth.
A Minimizer strat has to reach targets, so we use attractor construction. Then, analogue of Lemma Y proves that it is optimal. 

\subsection{Total reward}
Now we have the other Bellman equations, so Assumption (c) changes as follows.
Still, Lemma W holds. If there was a positive cycle, we anyway get inf reward. 

Then, depending on whether $\star=c$ or $\star=\infty$, we are in the reachability or safety analogue. 

\subsection{Mean payoff}
Following the strat that maximizes total reward eventually is optimal (cite sth?).
Both need attractor, as we could be stuck in a MEC that is bad for both.

\subsection{Summary}
Using attractor strategy, we are always eventually optimal. In some cases, it suffices to only follow optimal actions.

Maybe I can also have the general assumptions and then prove the Lemmata from those.



\section{Old stuff}

Concretely, we want to find a $\straa$ such that for all $\strab$:
$\pr_{\initstate}^{\straa,\strab}(\Diamond \fstates) = \val(\initstate)$.
Dually we also want a $\strab$ such that for all $\straa$: $\pr_{\initstate}^{\straa,\strab}(\Diamond \fstates) = \val(\initstate)$.
We start by proving it only for reachability. Afterwards we show how to generalize the proof to the other objectives.

Intuitively, in reachability for the Minimizer it suffices to just play actions which are optimal according $\ub$. For the Maximizer, we play optimally according to $\lb$, but additionally have to ensure that the actions make progress; we achieve this by only adding an action to the optimal set if it has a higher value than other actions, not, if it is equal. In the example, in the first iteration we add exit, as it is clearly better than the stay. In the second iteration we do not add stay, because it has the same value as exit. 

\subsection{Assumptions on the approximants}
We first state several assumptions which the approximants have to satisfy and for each assumption prove that it is satisfied for approximants coming from our algorithm. For ease of notation, we use the operator $\argopt$ to find the set of optimal actions for a state $\state$:
\[\argopt_{\action \in \Av(\state)} = \begin{cases}
	\argmax_{\action \in \Av(\mathsf{s})} &\mbox{ if } \state \in \maxstates\\
	\argmin_{\action \in \Av(\mathsf{s})} &\mbox{ if } \state \in \minstates
\end{cases}\]

\begin{itemize}
	\item the approximants are correct, i.e. for all states $\lb(\state) \leq \val(\state) \leq \ub(\state)$. This is assumption is satisfied for our algorithm by Theorem~\ref{BVIA_term}.
	
	\item the approximants are $\varepsilon$-close in the initial state, i.e. $\val(\initstate) - \lb(\initstate) < \varepsilon$ and $\ub(\initstate) - \val(\initstate) < \varepsilon$.
	This is satisfied for our algorithm, as the bounds are correct and the stopping criterion ensures $\ub(\initstate) - \lb(\initstate) < \varepsilon$.
	
	\item for all target states the lower approximant is 1.
	This assumption is satisfied by the initialization of the algorithm. 
	
	\item unfolding the Bellman equation for the approximants can only make them more precise, i.e. for all states $\state$:
	\[\lb(\state) \leq 
	\argopt_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \lb(\state')\]
	\[\ub(\state) \geq 
	\argopt_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \ub(\state')\]
	
	We first prove this assumption for the lower approximants.
	Let $i$ be the iteration in which the algorithm computing the approximants finished. We denote by $\lb<j>$ the approximants in the $j$-th iteration for all $j\leq i$.
	Then we have $\lb = \lb<i>$ by definition.
	The lower approximant is computed according to the Bellman equations \eqref{eq:Lsa} and \eqref{eq:Ls}. Thus for all states $\state$ we have 
	\begin{align*}
		\lb<i>(\state) &= 
		\argopt_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \lb<i-1>(\state') \\
		&\leq 
		\argopt_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \lb<i>(\state'),
	\end{align*}
	where the second inequality follows the fact that the bounds are monotonically increasing, i.e. $\lb<i-1>(\state) \leq \lb<i>(\state)$.
	
	For the upper approximant, the proof is mostly analogous, replacing $\leq$ with $\geq$. 
	However, we also have to address the additional deflating that can modify the upper approximants.
	If a state $\state$ is deflated down to $x$, then it is part of an EC $T$ and all states in the $T$ were deflated to $x$ as well. As $T$ is an EC, every $\state \in T$ has a staying action $\action<s>$. Since all successors of this action are in the EC and have an upper estimate of $x$, we have $\ub(\state,\action<s>) = x$. 
	Hence, if $\state$ is a  Minimizer state, we have $\ub(\state) = x$ and $\argmin_{\action' \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \ub(\state') \leq \ub(\state,\action<s>) = x$ and the assumption is satisfied.
	If $\state$ is a Maximizer state, we also use the fact that $x = \bE_{\ub}^{\Box}(T)$, and thus for all leaving actions $\action<\ell>$ we have $\ub(\state,\action<\ell>) \leq x$.
	Then, as all staying actions have an estimate of $x$ and all leaving actions have at most $x$, we can conclude that $\argmax_{\action' \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \ub(\state') = x$.	
	
	Note that given the true values $\val$, unfolding the Bellman equations for one step results in exactly the same values, as the value vector is a fixpoint. Thus, in that case we have an equality.
\end{itemize}

\subsection{Strategies following only the approximants}

Let $\sigL$ and $\tauU$ be the strategies that pick an action that is optimal according to the approximants $\lb$ respectively $\ub$.
Formally, for all states $\state$, let $\sigL(\state)$ be an element of $\argmax_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \lb(\state')$.
Dually, let $\tauU(\state)$ be an element of $\argmin_{\action \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \ub(\state')$.

We now prove that following these strategies for a finite number of steps does not decrease the probability to reach the target.
For this, let $\Diamond^{i} X \eqdef \{\path \in (\states \times \actions)^\omega \mid \path = \state_0 \action_0 \state_1 \action_1 \dots \wedge ~\state_i \in X\}$ denote the measurable set of all paths which reach the states $X \subseteq \states$ in exactly $i$ steps. Note that this definition only restricts a finite prefix of the path; however, as we have defined the probability distribution only over infinite paths, this set contains infinite paths.

\begin{lemma}[Following the approximants for a finite time]\label{lem:finiteFollow}
	For all states $\state \in \states$ and all $i \in \Naturals_0$, the following two statements hold:
	For all Minimizer strategies~$\strab$: 
	\[\sum_{\state' \in \states} \probability^{\sigL,\strab}_{\state}[\Diamond^i \{\state'\}] \cdot \lb(\state') \geq \lb(\state).
	\]
	Dually, for all Maximizer strategies $\straa$: 
	\[\sum_{\state' \in \states} \probability^{\straa,\tauU}_{\state}[\Diamond^i \{\state'\}] \cdot \ub(\state') \leq \ub(\state).
	\]
\end{lemma}
\begin{proof}
	We show only the first statement, as the second proof is completely analogous.
	We proceed by induction on $i$, the number of steps for which we follow~$\sigL$.
	For $i=0$, \[
	\probability^{\sigL,\strab}_{\state}[\Diamond^0 \{\state'\}] = \begin{cases}
		1 &\mbox{ if } \state=\state'\\
		0 &\mbox{ otherwise}
	\end{cases}.\]
	Thus, the left side of the inequality evaluates to $\lb(\state)$ and the base case is completed.
	
	For the induction step, the following chain of equations proves our goal. We justify every transformation below the equations.
	\begin{align*}
		&\sum_{\state' \in \states} \probability^{\sigL,\strab}_{\state}[\Diamond^{i+1} \{\state'\}] \cdot \lb(\state') \\
		&= \sum_{\state' \in \states} \probability^{\sigL,\strab}_{\state}[\Diamond^{i} \{\state'\}] \cdot \left( \sum_{t\in \states} \trans(\state',\pi(\state'),t) \cdot \lb(t) \right) \tag{Step 1}\\
		&\geq \sum_{\state' \in \states} \probability^{\sigL,\strab}_{\state}[\Diamond^{i} \{\state'\}] \cdot \lb(\state') \tag{Step 2}\\
		&\geq \lb(\state) \tag{Induction hypothesis}
	\end{align*}
	For Step 1, instead of considering paths that follow the strategies for $i+1$ steps, we consider paths that follow it for $i$ steps and explicitly unfold the final step. Here, $\pi(\state') = \begin{cases}
		\sigL(\state') &\mbox{ if } \state \in \maxstates\\
		\tau(\state') &\mbox{ if } \state \in \minstates
	\end{cases}$.
	
	For Step 2, we use the fourth assumption on the approximants, namely that unfolding the Bellman equation can only make them more precise. 
	If $\state'$ is a Maximizer state, by definition we have $\sigL(\state') = \argmax_{\action' \in \Av(\mathsf{s})} \sum_{\state' \in \states} \trans(\state,\action,\state') \cdot \lb(\state')$ and thus can immediately apply the assumption.
	If $\state'$ is a Minimizer state, we know that the assumption holds for $\argmin$ of all available actions, so it also holds for whichever action $\strab$ uses.
	In the final step, we apply the induction hypothesis.
	\qed
\end{proof}

\begin{lemma}\label{lem:tauU}
	$\tauU$ is an $\varepsilon$-optimal strategy of Minimizer.
\end{lemma}
\begin{proof}
	Using Lemma~\ref{lem:finiteFollow}, we have that for all states $\state$, all Maximizer strategies $\straa$ and all $i \in \Naturals_0$:
	\begin{align*}
		&\sum_{\state' \in \states} \probability^{\straa,\tauU}_{\state}[\Diamond^i \{\state'\}] \cdot \ub(\state') \\
		&=\left( \sum_{\state' \in \fstates} \probability^{\straa,\tauU}_{\state}[\Diamond^i \{\state'\}] \cdot \ub(\state')\right) + \left( \sum_{\state' \in \states \setminus \fstates} \probability^{\straa,\tauU}_{\state}[\Diamond^i \{\state'\}] \cdot \ub(\state') \right) \tag{Splitting the sum}\\
		&\leq \ub(\state) \tag{Lemma~\ref{lem:finiteFollow}}
	\end{align*}
	The second sum over all non-target states certainly evaluates to 0 or more. Also, $\ub(\state')=1$ for all $\state'\in\fstates$. Hence, it holds that 
	\[\sum_{\state' \in \fstates} \probability^{\straa,\tauU}_{\state}[\Diamond^i \{\state'\}] \leq \ub(\state).\]
	Thus, pulling the sum into the definition of the paths, we get
	\[\probability^{\straa,\tauU}_{\state}[\Diamond^i \fstates] \leq \ub(\state).\]
	Note that as this statement holds for all $i$ and all target states are absorbing, we can also take the limit and consider all paths that reach a target state $\Diamond \fstates$.
	Considering the initial state $\initstate$ and using that $\ub$ is correct and $\varepsilon$-optimal, we conclude that $\tauU$ is $\varepsilon$-optimal:
	\[\probability^{\straa,\tauU}_{\initstate}[\Diamond \fstates] \leq \ub(\initstate) \leq \val(\initstate) + \varepsilon.\]
\end{proof}

\subsection{Ensuring Maximizer makes progress}

We already saw in the counter-example in the beginning that the dual of Lemma~\ref{lem:tauU} is not true, as only playing actions according to the approximants is not $\varepsilon$-optimal.
We will now show how to augment $\sigL$ to become $\varepsilon$-optimal. 

We employ a folklore construction which is sometimes called \emph{attractor}, similar\footnote{In that paper, they ensure that the target or sink states are reached almost surely. We require that target states are reached with positive probability.} to the one used in~\cite[Section 5.3]{CAH13}.
In other words: we perform a backwards search from the target state, using only actions that are $\varepsilon$-optimal according to~$\lb$.

Formally, we use the following recursive procedure:
Let $\spanStates_0 = \fstates$.
For $i \geq 1$, we define 
\begin{align*}
	\spanStates_i &= \{\state \in \maxstates \mid \exists \action \in \argmax_{\action' \in \Av(\mathsf{s})} \lb(\state,\action'). \post(\state,\action) \cap \spanStates_{i-1} \neq \emptyset\}\\
	&\cup \{\state \in \minstates \mid \forall \action \in \Av(\state). \post(\state,\action) \cap \spanStates_{i-1} \neq \emptyset\}.
\end{align*} 
We terminate when $\spanStates_j = \spanStates_{j-1}$.

For all $i$, $\spanStates_i$ contains those states that have a path of length at most $i$ to the target which for Maximizer states uses only $\varepsilon$-optimal actions, and for Minimzer states has no other choice but to continue on a path towards the target. This can be proven by simple induction on the length of the path. 
Note that the states with no path to the target $\bot$ are not in $\spanStates_i$ for any $i$.

Let $\posVal \eqdef \{\state \in \states \mid \val(\state) > 0\}$ be all states with a positive value. As every state with a positive value has a path to a target state, it holds that $\posVal = \spanStates_j$, where $j$ is the iteration where the recursive procedure terminates.

We now define the $\varepsilon$-optimal Maximizer strategy $\sigLS$.
Note that for states in $\fstates$ or states with value 0, the strategy is irrelevant as either we anyway have reached target or no strategy can reach the target (against a rational opponent).
Thus, here $\sigLS$ picks an arbitrary available action.
For every state in $\state \in \posVal \setminus \fstates$, we pick an action as follows: 
let $i$ be the minimum number with $\state \in \spanStates_i$. As $\state\in\posVal$, such an $i$ exists.
Then the strategy $\sigLS(\state)$ picks an action from 
\[\{\action \in \Av(\state) \mid \action \in \argmax_{\action' \in \Av(\mathsf{s})} \lb(\state,\action') \wedge \post(\state,\action) \subseteq \spanStates_{i-1}\}.\]
Such an action exists, because $\state$ was added in the $i$-th step, hence it must have an action leading to $\spanStates_{i-1}$. Note that $i-1 \geq 0$, since $\state \notin \fstates$.

Under this strategy $\sigLS$, for every Minimizer strategy $\strab$, every state in $\state \in \posVal \setminus \fstates$ has a positive probability to reach the target states. To prove this, observe that every $\state$ is in some $\spanStates_i$. For a Maximizer state, by construction it uses an action with a positive chance to reach a state in $\spanStates_{i-1}$; for Minimizer, it has no choice but to put positive probability on reaching $\spanStates_{i-1}$. 
Repeating the argument until $i=0$ shows the claim.

\begin{lemma}
	$\sigLS$ is an $\varepsilon$-optimal strategy of Maximizer.
\end{lemma}
\begin{proof}
	We again use Lemma~\ref{lem:finiteFollow} and split the sum as in the proof of Lemma~\ref{lem:tauU}.
	However, this time we split $\states$ into $\fstates$, $\posVal$ and the remaining states with value 0. Note that for states with value 0 also the lower approximant is 0, since by assumption the lower approximant is correct. Hence, the summand considering the value 0 states evaluates to 0.
	Thus we have that for all states $\state$, all Minimizer strategies $\strab$ and all $i \in \Naturals_0$:
	\[
	\left( \sum_{\state' \in \fstates} \probability^{\sigLS,\strab}_{\state}[\Diamond^i \{\state'\}] \cdot \lb(\state')\right) + \left( \sum_{\state' \in \posVal \setminus \fstates} \probability^{\sigLS,\strab}_{\state}[\Diamond^i \{\state'\}] \cdot \lb(\state') \right) 
	\geq \lb(\state) 
	\]
	Here is the crucial difference between constructing a Maximizer and Minimizer strategy: For Maximizer, it is possible that the whole probability mass still remains in $\posVal$. Following a strategy that maximizes $\lb$ for a finite number of steps does not decrease the chance of reaching the targets, but it might be necessary to eventually switch to the optimal strategy in order to actually realize the value. 
	This is why we used the attractor construction to ensure that under $\sigLS$ every state in $\posVal \setminus \fstates$ has a positive probability to reach the target. 
	Then, for $i \to \infty$, the second summand converges to 0. Intuitively, more and more probability leaves towards the target or sink states. 
	Formally, as from every state there exists a path with positive probability to reach a target, the probability to reach $\fstates$ in $\abs{\states}$ steps is at least $q \eqdef p^{\abs{\states}}$, where $p$ is the minimum probability occurring in the SG. Since $\sum_i^\infty q \cdot (1-q)^i = 1$ (geometric series), the probability to remain in $\posVal \setminus \fstates$ is 0.
	
	Having ensured that the probability mass actually arrives at the target, we can consider the infinite behaviour and conclude:
	\[ \probability^{\sigLS,\strab}_{\state}[\Diamond \fstates]
	\geq \lb(\state)
	\]
	Note that we again pulled the sum into the definition of the paths and used that for target states the lower approximant is initialized to 1.
	Finally, considering the initial state and using that $\lb$ is correct and $\varepsilon$-close, we arrive at our goal:	
	\[\probability^{\sigLS,\strab}_{\initstate}[\Diamond \fstates]
	\geq \lb(\initstate) \geq \val(\initstate) - \varepsilon.\] 
	\qed
\end{proof}


Note that, given the true values $\val$, all inequalities in the proofs become equalities.
Thus, we also showed how to construct optimal strategies from the true value vector.
